A numerical study on reaction-induced radial fingering instability

The dynamics of $A + B \rightarrow C$ fronts is analyzed numerically in a radial geometry. We are interested to understand miscible fingering instabilities when the simple chemical reaction changes the viscosity of the fluid locally and a non-monotonic viscosity profile with a global maximum or minimum is formed. We consider viscosity-matched reactants $A$ and $B$ generating a product $C$ having different viscosity than the reactants. Depending on the effect of $C$ on the viscosity relative to the reactants, different viscous fingering (VF) patterns are captured which are in good qualitative agreement with the existing radial experiments. We have found that for a given chemical reaction rate, an unfavourable viscosity contrast is not always sufficient to trigger the instability. For every fixed $Pe$, these effects of chemical reaction on VF are summarized in the $Da-R_c$ parameter space that exhibits a stable region separating two unstable regions corresponding to the cases of more and less viscous product. Fixing $Pe$, we determine $Da$-dependent critical log-mobility ratios $R_c^+$ and $R_c^-$ such that no VF is observable whenever $R^-_c \leq R_c \leq R^+_c$. The effect of geometry is observable on the onset of instability, where we obtain significant differences from existing results in the rectilinear geometry.

==> macros.tex <==
%\newcommand{\R}{{\mathbb R}}
\def \Rp {R_c^+}
\def \t {t_{\rm on}}
\def \dissty {\displaystyle}
\def \K {\mathsfbi{K}}
\def \bn {\boldsymbol{n}}
\def \ra {\rightarrow}
\def \bv {\boldsymbol{v}}
\def \Omns {\Omega_{\rm noslip}}
\def \bU {\boldsymbol{U}}
\def \Omc {\Omega \backslash \Omega_{\rm noslip}}
\def \bx {\boldsymbol{x}}
\def \RR {\mathbb{R}}
\def \Rm {R_c^-}
\def \Rc {R_c}
\def \PA {Pe_A}
\def \Dc {\mathsfbi{D}_c}
\def \Dcm {\mathsfbi{D}_{c_m}}
\def \PB {Pe_B} 
\def \PC {Pe_C}
\def \Rcc {R_{c, {\rm crit}}}
\def \mcrit {\mu_{\rm crit}}
\def \Rb {R_b} 
\def \DC {D_C}
\def \DA {D_A}
\def \DB {D_B}
\def \mb {\mu_B}
\def \mc {\mu_C}
\def \ma {\mu_A}
\def \ms {\mu^{\ast}}
\def \bu {\boldsymbol{u}}
\def \upot {\boldsymbol{u}_{\rm pot}}
\def \urot {\boldsymbol{u}_{\rm rot}}
\def \pa {\partial}
\def \om {\omega} 
\def \rmn {r_{\rm min}} 
\def \rmx {r_{\rm max}} 
\def \ro {r_{\rm out}} 
\def \roo {r_{0, {\rm out}}}
\def \s {\sigma}
\def \a {\widetilde{a}}
\def \b {\widetilde{b}}
\def \c {\widetilde{c}}
\def \u {\widetilde{\bu}}
\def \p {\widetilde{p}}
\def \m {\widetilde{\mu}}
\def \rin {r_{\rm in}} 
%\def \r {r_{0, {\rm out}}} 
\def \R {\mathcal{R}}
\def \r {r_{0, {\rm in}}} 
\def \wt {\widetilde}
\def \dt {\wt{d}}
\def \ct {\wt{c}}
\def \tt {\wt{t}}
\def \htl {\wt{h}}
\def \G {\mathcal{G}}
\def \T {T_m}
\def \rl {\rho_l}
\def \rs {\rho_s}
\def \eb {\eta_b}
\def \s0 {\s_0}
%\def \s {\wt{\sigma}}
\def \M {\wt{M}_0}
\def \bseq {\begin{subequations}}
\def \eseq {\end{subequations}}
\def \bseqn {\begin{subeqnarray}}
\def \eseqn {\end{subeqnarray}}
\def \L {\Lambda}
\def \U {\mathcal{U}}
\def \Om {\Omega} 
\def \lap {\nabla^2} 
\def \beq {\begin{equation}}
\def \eeq {\end{equation}}
\def \bfig {\begin{figure}}
\def \efig {\end{figure}}
\def \beqn {\begin{eqnarray}}
\def \eeqn {\end{eqnarray}}
\def \k {\kappa}
\def \Lp {L^+}
\def \Lm {L^-}
\def \nn {\nonumber}
\def \al {\alpha}
\def \big0 {\mathcal{0}}
\renewcommand{\vector}[1]{(x_1,x_2,\ldots,x_{#1})}
%\newcommand{\D}[1]{\mathasfbi{D}_{#1}}
\newcommand{\avector}[2]{(#1_1,#1_2,\ldots,#1_{#2})}
\newcommand{\aDEFvector}[2][a]{(#1_1,#1_2,\ldots,#1_{#2})}
\newcommand{\abra}[1]{\left\langle #1\right\rangle}
\newcommand{\iv}[2]{#1^{(#2)}}
\newcommand{\ip}[2]{\left\langle #1, #2\right\rangle}
\newcommand{\bra}[1]{\left( #1 \right)}
\newcommand{\sqbra}[1]{\left[ #1 \right]}
\newcommand{\brac}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\normLLO}[1]{\left\lVert #1 \right\rVert_{L^2\bra{\Omega}}^2}
\newcommand{\LpLq}[2]{L^{#1}\bra{0, T; L^{#2}(\Om)}}
\newcommand{\grad}[1]{\bnabla #1}
\newcommand{\tgrad}[1]{\widetilde{\bnabla} #1}
\newcommand{\tdiv}[1]{\widetilde{\bnabla} \bcdot #1}
\newcommand{\divg}[1]{\bnabla \bcdot #1}
\newcommand{\norm}[1]{\left \lVert #1 \right \rVert}
\newcommand{\normLpO}[2]{\left\lVert #1 \right\rVert_{L^{#2}\bra{\Omega}}^{#2}}
\newcommand{\normLpq}[3]{\left\lVert #1 \right\rVert_{L^{#2}\bra{\Omega}}^{#3}}
\newcommand{\modu}[1]{\left\lvert #1 \right\rvert}
\newcommand{\crcl}{\raisebox{0.6pt}{\tikz{\node[draw,scale=0.5,circle,fill=none](){};}}}
\newcommand{\sqre}{\raisebox{0.5pt}{\tikz{\node[draw,scale=0.5,regular polygon, regular polygon sides=4,fill=none](){};}}}

